Neurosymbolic Transformers for Multi-Agent Communication

We study the problem of inferring communication structures that can solve cooperative multi-agent planning problems while minimizing the amount of communication. We quantify the amount of communication as the maximum degree of the communication graph; this metric captures settings where agents have limited bandwidth. Minimizing communication is challenging due to the combinatorial nature of both the decision space and the objective; for instance, we cannot solve this problem by training neural networks using gradient descent. We propose a novel algorithm that synthesizes a control policy that combines a programmatic communication policy used to generate the communication graph with a transformer policy network used to choose actions. Our algorithm first trains the transformer policy, which implicitly generates a "soft" communication graph; then, it synthesizes a programmatic communication policy that "hardens" this graph, forming a neurosymbolic transformer. Our experiments demonstrate how our approach can synthesize policies that generate low-degree communication graphs while maintaining near-optimal performance.

==> algo.tex <==

\begin{figure*}
\centering
\begin{minipage}{0.45\textwidth}
\begin{algorithm}[H]
\begin{algorithmic}
\Procedure{GetTrajectory}{$\pi,T$}
\State $\x_0\sim\istates$
\For{$t\in\{0,1,...,T-1\}$}
\State $\obs_t\gets h(\x_t)$
\For{$i\in[\nagents]$}
\State $\comm_t^i\gets\pi^\commVar(\x_t^i,\obs_t^i)$
\State $\mes_t^i\gets\{\pi^M(\x_t^j,\obs_t^{j,i})\mid j\in\comm_t^i\}$
\State $\act_t^i\gets\pi^\actionVar(\x_t^i,\obs_t^i,\mes_t^i)$
\EndFor
\State $\x_{t+1}\gets f(\x_t,\act_t)$
\EndFor
\State \Return $\x=(\x_0,\x_1,...,\x_T)$
\EndProcedure
\end{algorithmic}
\caption{Algorithm for sampling a trajectory from the decentralized POMDP.}
\label{alg:problem}
\end{algorithm}
\end{minipage}
\qquad
\begin{minipage}{0.45\textwidth}
\begin{algorithm}[H]
\begin{algorithmic}
\Procedure{TrainPolicy}{}
\State $\theta\gets\operatorname*{\arg\max}_{\theta'}J^\rewardVar(\pi_{\theta'})$
\State $P\gets\operatorname*{\arg\max}_P\tilde{J}(P;\theta)$
\State $\theta\gets\operatorname*{\arg\max}_{\theta'}J^\rewardVar(\pi_{{P,\theta'}})$
\State \Return $\pi_{P,\theta}$
\EndProcedure
\end{algorithmic}
\caption{Algorithm for training the multi-agent control policy.}
\label{alg:main}
\end{algorithm}
\end{minipage}
\end{figure*}


==> old_intro.tex <==
\section{Introduction}

Real-world robotics systems are often distributed in nature, with teams of agents needing to coordinate to share information and solve problems. Reinforcement learning has recently been demonstrated as a promising approach to automatically solve such multi-agent planning problems~\cite{tan1993multi,littman1994markov,foerster2016learning,lowe2017multi,foerster2018counterfactual,khan2019learning}.

A key challenge in (cooperative) multi-agent planning is how to coordinate with other agents, both deciding whom to communicate with and what information to share. One approach is to let agents communicate with all other agents; however, letting agents communicate arbitrarily can lead to poor generalization~\cite{khan2019graph,paulos2019decentralization}; furthermore, it cannot account for physical constraints such as limited bandwidth. A second approach is to manually impose a communication graph on the agents, typically based on distance~\cite{khan2019graph,tolstaya2019learning,paulos2019decentralization,shishika2020cooperative}. However, this manual structure may not reflect the optimal communication structure---for instance, one agent may prefer to communicate with another one that is farther away but in its desired path. A third approach is to use a transformer~\cite{vaswani2017attention} as the policy network~\cite{das2019tarmac}, which uses attention to choose which other agents to focus on. However, since the attention is soft, each agent still communicates with every other agent.

We study the problem of learning a communication policy that solves a multi-agent planning task while minimizing the amount of communication required. We measure the amount of communication on a given step as the maximum degree (in both directions) of the communication graph on that step; this metric captures the maximum amount of communication any single agent must perform at that step. While we focus on this metric, our approach easily extends to handling other metrics---e.g., the total number of edges in the communication graph, the maximum in-degree, and the maximum out-degree, as well as general combinations of these metrics.

The challenge with optimizing the maximum degree is that it is a global property of the communication graph. For instance, suppose each agent independently chooses whose information they want to receive; then, they may all choose to communicate with one agent that has highly desired information, but then this agent has very high degree in the communication graph. Thus, the agents must implicitly coordinate their decisions to minimize communication.

We propose an approach to addressing this problem. At a high level, our algorithm first trains a transformer policy for solving the multi-agent task; as described above, the soft attention weights capture the extent to which an edge in the communication graph is useful. Next, our algorithm trains a communication policy that optimizes both goals: (i) match the transformer as closely possible, and (ii) minimize the maximum degree of the communication graph at each step. In contrast to the transformer policy, this communication policy makes hard decisions about which other agents to communicate with. Finally, our algorithm re-trains the weights of the transformer policy, except where the (hard) attention weights are chosen by the communication policy.

A key question is how to train the communication policy. Training a neural network policy is hard since the maximum degree of the communication graph is a discrete objective that cannot be optimized using gradient descent. An alternative is to train a structured model such as a decision tree~\cite{breiman1984classification} or rule list~\cite{wang2015falling} using combinatorial optimization. However, these models perform poorly since choosing whom to communicate with requires reasoning over sets of other agents---e.g., to avoid collisions, an agent must communicate with its nearest neighbor in its direction of travel.
%\david{remove}

Instead, our algorithm synthesizes \emph{programmatic} communication policies; in contrast to rule lists, these polices include components such as filter and map that operate over sets of inputs. In particular, we define a domain-specific language (DSL) encoding programs that each select a fixed number of other agents to communicate with. Then, we use a stochastic synthesis algorithm~\cite{schkufza2013stochastic} based on MCMC sampling~\cite{metropolis1953equation,hastings1970monte} to synthesize programs that optimize both objectives (i) and (ii) above.

In addition to standard list-processing components, an important construct in our DSL is a random choice operator. Intuitively, random choice is a key ingredient needed to minimize the communication graph degree without global coordination. For example, if suppose there are two groups of agents, and each agent in group $A$ needs to communicate with an agent in group $B$, but the specific one does not matter. Using a deterministic communication policy, each agent in group $A$ might choose to communicate with the same agent in group $B$ (assuming it is hard for the policy distinguish agents within a group). In contrast, having each agent in group $A$ communicate with a uniformly random agent in group $B$ provides a near-optimal solution to this problem.

We evaluate our approach on several multi-agent planning tasks that require agents to coordinate to achieve their goals. We demonstrate that our algorithm learns communication policies that  achieve task performance similar to the original transformer policy (i.e., where each agent communicates with every other agent), while significantly reducing the amount of communication. Our results demonstrate that our algorithm is a promising approach for training policies for multi-agent systems that additionally optimize combinatorial properties of the communication graph.

\begin{figure}
\centering
\includegraphics[width=0.32\textwidth]{01_traj.pdf}
\includegraphics[width=0.32\textwidth]{2g_tf-attn.pdf}
\includegraphics[width=0.32\textwidth]{2g_prog-retrained-attn.pdf}
\caption{Left: Two groups of agents (red vs. blue) at their initial positions (circles) trying to reach their goal positions (crosses). Agents must communicate both within group and across groups to choose a collision free path to take (solid line shows a path for a single agent in each group). Middle: The soft attention weights of the transformer policy computed by the agent along the $y$-axis for the message received from the agent along the $x$-axis for the initial step. Group 1 attends to messages from all agents, whereas Group 2 only attends to messages from Group 1. Right: The hard attentions learned by the programmatic communication policy to imitate the transformer.}
    \label{fig:run_ex}
\end{figure}
\textbf{Example.}
%
Consider the example in Figure~\ref{fig:run_ex}, where agents in group $1$ (blue) are navigating from the left to their goal on the right, while agents in group $2$ (red) are navigating from the right to their goal on the left. In this example, agents have noisy observations of the positions other agents (e.g., based on cameras or LIDAR); however, they do not have access to internal information such as their planned trajectories or even their goals.
%The presence of each group is sampled randomly and the goal is to learn a single (decentralized) policy for all the settings.
Thus, to solve this task, each agent must communicate both with its closest neighbor in the same group (to avoid colliding with them), as well as with any agent in the opposite group (to coordinate so their trajectories so they do not collide). The communication graph of the transformer policy is shown in Figure~\ref{fig:run_ex} (middle); as can be seen, the graph is not too dense, but it nevertheless has high degree since every agent in group $1$ communicates with every agent in group $2$ and vice versa. The programmatic communication policy synthesized by our algorithm is
\begin{align*}
\text{argmax}(\text{map}(-d^{i,j}, \text{filter}(\theta^{i,j} \ge -1.85, l))),\qquad
\text{random}(\text{filter}(d^{i,j} \ge 3.41, l)).
\end{align*}
Agent $i$ uses this program to choose two other agents $j$ from the list of agents $\ell$ from whom to request information; $d^{i,j}$ is the distance between them and $\theta^{i,j}$ is the angle between them. The first rule chooses the nearest agent $j$ (besides itself) such that $\theta^{i,j}\in[-1.85, 3.14]$, and the second chooses a random agent in the other group. The communication graph is visualized in Figure~\ref{fig:run_ex} (right).
%\david{Change the description}

%For the example in Figure~\ref{fig:run_ex}, the feature map $\phi(\x^i, \obs^{i,j})$ is the vector $[x^g, y^g, d^g, \theta^g, x^r, y^r, d^r, \theta^r]$ where $(x^g, y^g)$ (resp., $(x^r,y^r)$) is the agent's relative position to its goal (resp., other agent), $d^g$ (resp., $d^r$) is the distance to the goal (resp., other agent) and $\theta^g$ (resp., $\theta^r$) is the angle of the relative position to the goal (resp., other agent) with respect to the x-axis. The programmatic communication policy learned has the following rules--(i)  which chooses a random agent in the other group. For this example, we forced the weights $\beta$ to be non-zero for at most one feature to improve the interpretability of the rules. This constraint is not used for the results in Section~\ref{sec:experiments}.


%\textbf{Contributions.}
%
%We formulate the problem of learning the communication structure for a multi-agent planning problem (Section~\ref{sec:problem}), propose an algorithm for solving this problem by synthesizing a programmatic communication policy to mimic an oracle based on the transformer architecture (Section~\ref{sec:approach}), and experimentally demonstrate the benefits of our approach (Section~\ref{sec:experiments}).

\textbf{Related work.}
%
There has been a great deal of recent interest in using reinforcement learning to automatically infer good communication structures for solving multi-agent planning problems~\cite{khan2019graph,tolstaya2019learning,paulos2019decentralization,das2019tarmac,shishika2020cooperative}. Much of this work focuses on inferring what to communicate rather than whom to communicate with; they handcraft the communication structure to be a graph (typically based on distance)~\cite{khan2019graph,tolstaya2019learning,paulos2019decentralization}, and then use a graph neural network~\cite{scarselli2008graph,kipf2016semi} as the policy network. There has been some prior work using transformer network to infer the communication graph~\cite{das2019tarmac}; however, they rely on soft attention, so the communication graph remains fully connected.

There has also been a great deal of interest using an oracle (in our case, the transformer policy) to train a policy (in our case, the programmatic communication policy)~\cite{levine2013guided,montgomery2016guided}. In the context of multi-agent planning, this approach has been used to train a decentralized control policy using a centralized one~\cite{tolstaya2019learning}; however, their communication structure is manually designed.

Finally, in the direction of program synthesis, there has been much recent interest in leveraging program synthesis in the context of machine learning~\cite{ellis2015unsupervised,ellis2018learning,valkov2018houdini,pu2018selecting,young2019learning,liu2019learning}. Specifically in the context of reinforcement learning, it has been used to synthesize programmatic control policies that are more interpretable~\cite{verma2018programmatically,verma2019imitation}, that easier to formally verify~\cite{bastani2018verifiable,sadraddini2019polytopic}, or that generalize better~\cite{inala2020synthesizing}; to the best of our knowledge, none of these approaches have considered multi-agent planning problems.



%An added benefit of using programmatic rules for communication is interpretability [and generalizability, verifiability.]

%[Compare to prior work - almost same but query, key and value also depend on relative features ]

